AOMD: An Analogy-aware Approach to Offensive Meme Detection on Social Media

This paper focuses on an important problem of detecting offensive analogy meme on online social media where the visual content and the texts/captions of the meme together make an analogy to convey the offensive information. Existing offensive meme detection solutions often ignore the implicit relation between the visual and textual contents of the meme and are insufficient to identify the offensive analogy memes. Two important challenges exist in accurately detecting the offensive analogy memes: i) it is not trivial to capture the analogy that is often implicitly conveyed by a meme; ii) it is also challenging to effectively align the complex analogy across different data modalities in a meme. To address the above challenges, we develop a deep learning based Analogy-aware Offensive Meme Detection (AOMD) framework to learn the implicit analogy from the multi-modal contents of the meme and effectively detect offensive analogy memes. We evaluate AOMD on two real-world datasets from online social media. Evaluation results show that AOMD achieves significant performance gains compared to state-of-the-art baselines by detecting offensive analogy memes more accurately.

==> note.tex <==
Guideline
https://www.elsevier.com/journals/information-processing-and-management/0306-4573/guide-for-authors

TODO:

[x] Cover Letter: If your submission is based on prior published research, the cover letter is the reasonable medium to fully disclose the previous publication(s) of the manuscript or any portion of the manuscript and the level of copyright.

[ ] Recommended Reviewers: Authors are required to recommend at least 5 international reviewers from a mixture of countries and institutions. These recommended reviewers must be published in the research area, with no conflicts. Authors must provide institutions, institution email addresses, and reasons for recommending. Note: There is a possibility that IP&M may have to reject your manuscript if we are unable to find enough reviewers after a reasonable period.

[x] Title Page: With the title, author names, and affiliations. Present the authors' affiliation addresses (where the actual work was done) below the names. Indicate all affiliations after the author's name and in front of the appropriate address. Provide the postal address of each affiliation, including the country name, and the e-mail address of each author. Indicate who is the corresponding author.

[not required at this moment] 
Highlights: Highlights consist of a short collection of bullet points that capture the novel results of your research. Please have a look at the examples here: example Highlights. Highlights should include 3 to 5 bullet points (maximum 85 characters, including spaces, per bullet point).


* We study a novel problem of detecting offensive analogy memes on online social media.
* We design a principled scheme to jointly exploit multi-modal content in meme posts.
* We explicitly model the relations between visual and textual content in memes.
* We collect two real-world datasets to evaluate the detection performance. 
* Evaluation results show significant performance gains of the proposed solution.
% * The proposed solution outperforms state-of-the-art baselines in accurately detecting offensive analogy memes.


% - Not part of editorial consideration and aren't required until the final files stage
% - Only required for full research articles
% - Must be provided as a Word document— select "Highlights" from the drop-down list when uploading files
% - Each Highlight can be no more than 85 characters, including spaces
% - No jargon, acronyms, or abbreviations: aim for a general audience and use keywords
% - Consider the reader - Highlights are the first thing they'll see



[x] Manuscript: The manuscript must include a maximum of 6 keywords, all figures (including relevant captions), all tables (including titles, description, footnotes). Authors are required to obtain a copyright for material within their submission. Ensure the manuscript has been spell-checked and grammar-checked. Ensure all references mentioned in the reference list are cited in the text, and vice versa.

[ ] Competing Interests Statement: A competing interests statement is provided, even if the authors have no competing interests to declare.

[x] Author contributions: For transparency, authors are to submit an author statement file outlining their contributions to the paper using the relevant CRediT roles: Conceptualization; Data curation; Formal analysis; Funding acquisition; Investigation; Methodology; Project administration; Resources; Software; Supervision; Validation; Visualization; Roles/Writing - original draft; Writing - review & editing. Authorship statements should be formatted with the names of authors first and CRediT role(s) following. More details and an example.




Elsevier policy for arXiv
https://www.elsevier.com/about/policies/sharing

